Text2Chart: A Multi-Staged Chart Generator from Natural Language Text

Generation of scientific visualization from analytical natural language text is a challenging task. In this paper, we propose Text2Chart, a multi-staged chart generator method. Text2Chart takes natural language text as input and produce visualization as two-dimensional charts. Text2Chart approaches the problem in three stages. Firstly, it identifies the axis elements of a chart from the given text known as x and y entities. Then it finds a mapping of x-entities with its corresponding y-entities. Next, it generates a chart type suitable for the given text: bar, line or pie. Combination of these three stages is capable of generating visualization from the given analytical text. We have also constructed a dataset for this problem. Experiments show that Text2Chart achieves best performances with BERT based encodings with LSTM models in the first stage to label x and y entities, Random Forest classifier for the mapping stage and fastText embedding with LSTM for the chart type prediction. In our experiments, all the stages show satisfactory results and effectiveness considering formation of charts from analytical text, achieving a commendable overall performance.

==> results.tex <==
\section{Experimental Analysis (old)\label{secResOld}}
\begin{comment}

The overall experiment of our technique is divided into three parts - 1. The construction of our dataset, 2. Evaluation Metrics and 3. Results and Discussion.
\subsection{Dataset Construction} 
For the automatic generation of a chart out of a natural language text, our work requires a dataset from which the text samples are suitable for recognizing the chart information.  Here chart information refers to the x-axis entities and the corresponding y-axis values respectively.  The text samples must contain all these entities to build the particular chart.  Due to the unavailability of such a dataset, indeed we have prioritized in making our own dataset. Therefore, we ensure the format for the text sample of our dataset to be less complex, from where chart information can be recognized easily to create suitable charts subsequently. To collect such text samples, we have used online articles such as; Wikipedia, Live Science, Daily Star, and other statistics websites. We have also asked volunteers to write the suitable text samples that can be converted into a chart. They were given the freedom to write out of any context they wanted. From these resources we have managed to collect 717 text samples in total consisting of 30027 words, with the average length of 53 words, and the maximum length of 303 words. After performing appropriate and required labelling for each stage of our technique, we split our dataset as 464: 116: 137 text samples for training: validation: test sets. The number of instances of stage 1, 2 and stage 3 is shown in table \ref{instances}.

\begin{table}[ht]
\caption{The number of instances of stage 1, 2 and 3 for training, validation and test sets.}
\footnotesize
\centering
\begin{tabular}{p{1.6cm}|p{1.2cm}|p{1.3cm}|p{1.3cm}|p{1.3cm}|p{1.3cm}|p{1.2cm}|p{0.6cm}|p{0.6cm}}
    \hline
    &&\multicolumn{4}{c}{Stage 1}&Stage\,2&\multicolumn{2}{c}{Stage 3}\\ \hline
    &Sample&X Token Count&Y Token Count&X label Instance&Y label Instance& Map&pie&line\\ \hline
    Training &464&3411	&3614	&1984	&1909	&1984	&73	&58\\
    Validation&116&985	&1058	&548	&529	&548	&20	&11\\
    Test&137&988	&1075	&574	&561	&574	&20	&15
\end{tabular}
\label{instances}
\end{table}
 

\subsection{Evaluation Metrics}
As our technique is multi-staged, we adopt several different evaluation metrics for each stage in order to evaluate the performance of our work. For stage 1, we adopt the f1-score and its variants (e.g. macro-average F1-score, harmonic mean of f1-scores etc.). We observe the Receiver Operating Characteristic (ROC) curve and the area under curve (AUC-ROC) in order to summarize the curves and compare classifiers in the second stage. Finally for stage 3, we adopt Matthews correlation coefficient (MCC) evaluation metric, as for the MCC being a more reliable statistical rate than F1-score and accuracy in binary classification evaluation for imbalanced dataset \cite{chicco2020advantages}.


\subsection{Results and Discussion}
We discuss the results of each experiment for all the stages of our work here. Then we describe the overall performance of each stage and hold a complete discussion at the end.

\subsubsection{Experimental Analysis of Stage 1:}
The first stage of our work is x-axis and y-axis label entity recognition. Here we predict whether a given word from the text input can be an x-axis or y-axis entity. We experiment with our model combining several models, such as fastText, Word2Vec and BERT+LSTM in order to recognize these entities.

\textbf{Stage 1 Results using fastText:} At first, we train the fastText model for recognizing the x-axis and y-axis entities from a given text input separately. Then we combine the model for both the x and y-axis entity recognition task. We run our model on the training and validation sets while setting the number of epochs and batch size to 8. We have also used five layers of neuron units (i.e., 512L, 128L, 64T, 1024D, 3D) and tf random seed and numpy random seed to 139 and 141 respectively. This configuration has been set to measure the performance of our model using fastText for the x and y-axis entity recognition task, both separately and combined. We have obtained best results for x-entity recognition by setting the sequence length to 100. For the y-entity recognition and x and y-entity recognition (combined) tasks, the sequence length has been set to 55 for the best results.

\paragraph{\textbf{FastText for X-entity Recognition:}} Results of the x-entity recognition task using fastText model have been shown in table \ref{fx_1}. Here we get a score of above or equal to 0.80 and 0.64 of precision, recall and f1-score for positive classes in train and validation sets respectively. Here, positive class refers to the entities that have successfully got recognized by our model. We also calculate the macro-average and the harmonic mean of f1-score which is 0.88 and 0.87 in the training set and 0.79 and 0.77 in the validation set respectively.

\begin{table}[!htb]
\caption{Stage 1 results of training and validation set for x-entity recognition using fastText model.}
\label{fx_1}
\footnotesize
\centering
\begin{tabular}{p{0.8cm}p{1.6cm}p{1.3cm}p{1.3cm}p{1.3cm}}
    &&Precision (X) &Recall (X) &F1-score (X)\\ \hline
    \multicolumn{1}{c}{\multirow{4}{*}{x-entity recognition}}&Training set&0.81&0.80&0.80\\
    \multicolumn{1}{c}{}&Validation set&0.68&0.64&0.66\\ \hline
\end{tabular}
\end{table}

\begin{table}[!htb]
\caption{Stage 1 results based on harmonic mean f1-score using FastText and Word2Vec model.}
\label{h_mean_Fast_w2v}
\footnotesize
\centering
\begin{tabular}{|c|c|c|c|}
    Model &F1-score (X)&F1-score (Y) &Harmonic mean of F1-score \\ \hline
    \multirow{2}{*}{FastText}&0.8&0.9&0.8470588235\\
	&0.66&0.85&0.7430463576 \\ \hline
    \multirow{2}{*}{Word2Vec}&0.89&	1&	0.9417989418\\
	&0.67&	0.78&	0.7208275862 \\ \hline
\end{tabular}
\end{table}

\begin{table}[!htb]
\caption{Stage 1 results of training and validation set for y-entity recognition task using fastText model.}
\label{fx_2}
\footnotesize
\centering
\begin{tabular}{p{0.8cm}p{1.6cm}p{1.3cm}p{1.3cm}p{1.3cm}}
    &&Precision (Y) &Recall (Y) &F1-score (Y)\\ \hline
    \multicolumn{1}{c}{\multirow{4}{*}{y-entity\, recognition}}&Training set&0.93&0.88&0.90\\
    \multicolumn{1}{c}{}&Validation set&0.89&0.81&0.85\\
\end{tabular}
\end{table}

\paragraph{\textbf{FastText for Y-entity Recognition:}} We evaluate the results of the y-entity recognition task using FastText model as same as x-entity recognition task, shown in table \ref{fx_2}. Then we obtain 0.93, 0.88 and 0.9 of precision, recall and f1-score respectively for positive class in the train set. For the validation set the score is 0.89, 0.81 and 0.85. Here, the macro-average f1-score is 0.94 and 0.91 in the training and validation set respectively and the harmonic mean of f1-score is no different.

\paragraph{\textbf{FastText (Combined):}}
After training our model using fastText for x and y-entity recognition tasks separately, we combine the model in order to recognize both the x and y-axis entities together. Here we use the five layers of neuron units as  (i.e., 512L, 128L, 64T, 1024D, 4D) and the other configuration remains the same. Table \ref{fx} shows the results of the train and validation set for the combined x and y-entity recognition task. Here, the precision, recall and f1-score have been given for the positive classes of x and y-entities, for instance, precision(1) means precision of positive class of x-entity recognition and precision(2) means precision of positive class of y-entity recognition. We obtain a macro-average f1-score of 0.88 and 0.82 and the harmonic mean of f1-score of 0.84 and 0.76 in the train and validation set respectively.

\begin{table}[!htb]
\caption{Stage 1 results of training and validation set for x and y-entity recognition (combined) using fastText model.}
\label{fx}
\footnotesize
\centering
\begin{tabular}{p{1.5cm}p{1.3cm}p{1.3cm}p{1cm}p{1cm}p{0.9cm}p{0.9cm}p{1.4cm}}
    &Precision (X)&Precision (Y)&Recall (X)&Recall (Y) &F1-score (X)&F1-score (Y)&Harmonic mean of\,F1-score \\ \hline
    Training set&0.81&0.89&0.73&0.97&0.77&0.93&0.84\\ \hline
    Validation set&0.73&0.86&0.60&0.93&0.66&0.89&0.76\\ \hline
\end{tabular}
\end{table}

\textbf{Stage 1 Results using word2vec:}
The mechanism of word2vec concedes words of a corpus, sharing common context to locate in the close neighborhood in the vector space. Therefore we use Word2Vec in our model in order to assign each word of our corpus into the vector space where words are closely located to its related words. We first train our model to recognize x and y-entities separately then combine the model to recognize both x and y-entities at the same time using the word2vec model as well,  same as the fastText model.

\paragraph{\textbf{Word2Vec for X-entity Recognition:}}
For x-entity recognition using word2vec, we set the text sequence length to 100, number of epochs to 16 and batch size to 8. We use five layers of neuron units - 512L, 128L, 64T, 1024D, 3D and the numpy random and tf random seeds are set to 187 and 191 respectively. Table \ref{w2v_1} shows the results of x-entity recognition for the train and validation set where we achieve the f1-score for positive class of 0.89 and 0.67 respectively. The macro average f1-score for the training set is 0.93 and 0.80 for the validation set. We achieve the harmonic mean of f1-score of 0.93 and 0.78 for train and validation set respectively which is much better than the fastText model.

\begin{table}[!htb]
\caption{Stage 1 results of training and validation set for x-entity recognition using word2vec model.}
\label{w2v_1}
\footnotesize
\centering
\begin{tabular}{p{0.8cm}p{1.6cm}p{1.3cm}p{1.3cm}p{1.3cm}}
    &&Precision (X) &Recall (X) &F1-score (X) \\ \hline
    \multicolumn{1}{c}{\multirow{4}{*}{x-entity recognition}}&Training set&0.90&0.88&0.89\\
    \multicolumn{1}{c}{}&Validation set&0.72&0.62&0.67\\ \hline
\end{tabular}
\end{table}

\begin{table}[!htb]
\caption{Stage 1 results of training and validation set for y-entity recognition using word2vec model.}
\label{w2v_2}
\footnotesize
\centering
\begin{tabular}{p{0.8cm}p{1.6cm}p{1.3cm}p{1.3cm}p{1.3cm}}
    &&Precision (Y) &Recall (Y) &F1-score (Y) \\ \hline
    \multicolumn{1}{c}{\multirow{4}{*}{y-entity\, recognition}}&Training set&1&1&1\\
    \multicolumn{1}{c}{}&Validation set&0.79&0.77&0.78\\
\end{tabular}
\end{table}

\paragraph{\textbf{Word2Vec for Y-entity Recognition:}}
For y-entity recognition task, we obtain the best results using word2vec model while setting the text sequence length to 200 and number of epochs to 50. The number of layers, neuron units, seeds and batch size remains the same as the x-entity recognition task (512L, 128L, 64T, 1024D, 3D). The results of y-entity recognition using word2vec is shown in table \ref{w2v_2}. Although we have achieved 100\% f1-score in the train set, in the validation set the score is only 78\% which is less than the fastText model.

\paragraph{\textbf{Word2Vec (Combined):}}
We set the text sequence length to 100, batch size to 1, np and tf seeds to 141 and 139 respectively for the combined x and y-entity recognition task using word2vec model. The number of neuron units remains the same as 512L, 128L, 64T, 1024D, 4D. We train the model for sixty epochs and gain the best results using this model, shown in table \ref{w2v}. Here we achieve the macro-average  f1-score of 1.0 in the training set, but 0.78 in the validation set. Thus we take into consideration that the results achieved using the word2vec model are not better than the results achieved using the fastText model for stage 1.

\begin{table}[!htb]
\caption{Stage 1 results of training and validation set for x and y-entity recognition (combined) using word2vec model.}
\label{w2v}
\footnotesize
\centering
\begin{tabular}{p{1.5cm}p{1.3cm}p{1.3cm}p{0.8cm}p{0.8cm}p{0.9cm}p{0.9cm}p{1.0cm}}
    &Precision (X)&Precision (Y)&Recall (X)&Recall (Y) &F1-score (X)&F1-score (Y)&Harmonic mean of\,F1-score \\ \hline
    Training set&0.99&1.0&0.99&1.0&0.99&1.0&0.995\\ \hline
    Validation set&0.72&0.83&0.64&0.74&0.68&0.78&0.73\\ 
\end{tabular}
\end{table}

\textbf{Stage 1 Results using BERT+LSTM: }
Here we use the combination of BERT and LSTM to train our model for the x-entity and y-entity recognition task both individually and combined.

\paragraph{\textbf{BERT+LSTM for X-entity Recognition:}}
For x-entity recognition task, we set the sequence length to 30, number of epochs to 80, batch size to 2, np and tf seeds to 187 and 191 respectively. We use five layers of neuron units such as, 1024L, 1024L, 1024T, 256D, 4D. Table \ref{bl_1} shows the results of x-entity recognition using BERT+LSTM where we obtain the f1-score of 0.998 and 0.876 in the train and validation set respectively. These obtained results \ref{bl_1} are the best so far for x-entity recognition. 

\begin{table}[!htb]
\caption{Stage 1 results of training and validation set for x-entity recognition using BERT+LSTM model.}
\label{bl_1}
%\footnotesize
\centering
\begin{tabular}{p{0.8cm}cccc}
    &&Precision(X) &Recall(X) &F1-score(X)\\ \hline
    \multicolumn{1}{c}{\multirow{2}{*}{x-entity recognition}}&Training set&0.9974&0.999&0.998\\
    \multicolumn{1}{c}{}&Validation set&0.89&0.86&0.876\\ \hline
\end{tabular}
\end{table}

\begin{table}[!htb]
\caption{Stage 1 results of training and validation set for y-entity recognition using BERT+LSTM model.}
\label{bl_2}
%\footnotesize
\centering
\begin{tabular}{p{0.8cm}cccc}
    &&Precision(Y) &Recall(Y) &F1-score(Y)\\ \hline
    \multicolumn{1}{c}{\multirow{2}{*}{y-entity\, recognition}}&Training set&0.996&0.999&0.997\\
    \multicolumn{1}{c}{}&Validation set&0.956&0.988&0.972\\
\end{tabular}
\end{table}

\paragraph{\textbf{BERT+LSTM for Y-entity Recognition:}}
We achieve best results for y-entity recognition using BERT+LSTM while setting the text sequence length to 500, batch size to 8 and the seeds are as same as x-entity recognition. Here we use six layers of neuron units - 1024L, 1024L, 1024T, 256D, 256D, 4D. We run this model for only three epochs and obtain the results shown in table \ref{bl_2}. We have achieved the f1-score of 0.997 and 0.972 in the train and validation set respectively. Thus we deem that our model works better using the BERT+LSTM than using FastText for the y-entity recognition task as well.

\paragraph{\textbf{BERT+LSTM (Combined):}}
For the combined x and y-entity recognition task we use five layers of neuron units - 1024L, 1024L, 1024T, 1024D, 5D. We set the sequence length to 100, batch size to 1, np and tf seeds to 187 and 191 respectively. From table \ref{bl}, we obtain the macro-average f1-score of  0.99 and 0.92 in the train and validation set respectively. Our model for the combined x and y-entity recognition task using BERT+LSTM outperforms FastText and Word2Vec models. Therefore we continue using BERT+LSTM to test our corpus and evaluate the model performance in the final results of stage 1.

\begin{table}[!htb]
\caption{Stage 1 results of training and validation set for x and y-entity recognition (combined) using BERT+LSTM model.}
\label{bl}
\footnotesize
\centering
\begin{tabular}{p{1.5cm}p{1.3cm}p{1.3cm}p{0.8cm}p{0.8cm}p{0.9cm}p{0.9cm}p{1.0cm}}
    &Precision (X)&Precision (Y)&Recall (X)&Recall (Y) &F1-score (X)&F1-score (Y)&Harmonic mean of\,F1-score \\ \hline
    Training set&0.99&0.99&1.0&1.0&0.99&0.99&0.99\\ \hline
    Validation set&0.86&0.96&0.78&0.97&0.82&0.97&0.89\\ \hline
\end{tabular}
\end{table}

\textbf{Final Results of Stage 1: }
We have experimented our model using FastText, Word2Vec and BERT+LSTM for sub-task 1 where BERT+LSTM shows outstanding results among them. Thus we run our model on the test set using BERT+LSTM. The final results of stage 1 are shown in table \ref{1_final} where we also show the confusion matrix for the train, validation and test sets. Here we achieve the f1-score of 0.84 for x-entity recognition and 0.97 for y-entity recognition in the test set. The harmonic mean of f1-score is 0.998, 0.92 and 0.899 in the train, validation and test set respectively shown in table \ref{1_final_hmean}. Our experimental results show that our model using BERT+LSTM performs better than the other and can be reused in the stage 2 to utilize its availed knowledge. 

\begin{table}[!htb]
\caption{The final results of stage 1 including the confusion matrix of training, validation and test set using BERT+LSTM model.}
\label{1_final}
\footnotesize
\centering
\begin{tabular}{ccp{0.7cm}p{0.7cm}p{0.7cm}p{0.7cm}ccp{1.2cm}}
    &&TN (0,0) &FP (0,1)&FN (1,0)&TP (1,1)&Precision&Recall&F1-score\\ \hline
    \multicolumn{1}{c}{\multirow{3}{*}{BERT+LSTM(X)}}&Training set&22365&9&5&3406&0.997&0.999&0.998\\
    \multicolumn{1}{c}{}&Validation set&5718&101&138&847&0.89&0.86&0.88\\
    \multicolumn{1}{c}{}&Test set&6079&143&178&810&0.85&0.82&0.84\\ \hline
    \multicolumn{1}{c}{\multirow{3}{*}{BERT+LSTM(Y)}}&Training set&22158&14&5&3608&0.996&0.999&0.997\\
    \multicolumn{1}{c}{}&Validation set&5698&48&13&1045&0.96&0.99&0.97\\
    \multicolumn{1}{c}{}&Test set&6094&41&17&1058&0.96&0.984&0.97\\
\end{tabular}
\end{table}

\begin{table}[!htb]
\caption{The final results of stage 1 for the x and y-axis entity recognition (individual) task using BERT+LSTM.}
\label{1_final_hmean}
%\footnotesize
\centering
\begin{tabular}{cp{3.5cm}p{3.5cm}p{2.8cm}}
    &F1-score\,of BERT+LSTM(X)&F1-score\,of BERT+LSTM(Y)&Harmonic\, mean of F1-score \\ \hline
    Training set&0.9979490185&0.997373877&0.9976613648\\ \hline
    Validation set&0.8763579928&0.9716410972&0.9215431395\\ \hline
    Test set&0.8346213292&0.9733210672&0.8986508911\\ \hline
\end{tabular}
\end{table}


\subsubsection{Experimental Analysis of Stage 2: }
 Here we analyze the results of stage 2 that is mapping each of the x-axis entities with its corresponding y-axis value. We have run several experiments on our dataset, where 47 samples out of 717 contain inequality among x and y entities: a. Transfer model - with the combination of BERT and LSTM, b. Probability distribution - excluding and including punctuations, and c. X-X Distance and X-Y Displacement. After comparing these models, we evaluate the best performing model to run our test set in order to calculate the final results for stage 2.

\textbf{Transfer model: }
We reuse the BERT+LSTM (individual) model, the best model of stage 1 to utilize its gained knowledge in the stage 2 in order to enhance generalization about each task. Using BERT embedding and LSTM, we run two individual models, BERT+LSTM (X) and BERT+LSTM (Y). The number of hidden layers are eight in total, four layers each for x-axis entities and y-axis values. We configure both the model equally with batch size = 1, number of epochs = 8, LSTM layer 1024, 1024 and dense layer 256, 256. Then we run the model on training instances containing 8346 positive and 1973 negative instances and validation instances containing 3026 positive and 548 negative instances. Finally, we measure the model performance in terms of F1-score and AUC evaluation metrics. Results \ref{transfer_tab} show that the model BERT+LSTM (Y) underperforms in all of its hidden layers providing zero F1-score. Therefore, we have tried to improve the performance in our further experiments using different models. 

\begin{table}[!htb]
\caption{Stage 2 results of the Transfer Model in terms of F1-score and AUC}
\label{transfer_tab}
\centering
\begin{tabular}{|c|c|c|} \hline
    Model &F1-score &AUC \\ \hline
    Bert LSTM (X) layer 1 &0.41 &0.64 \\ \hline
    Bert LSTM (X) layer 2 &0.38 &0.62 \\ \hline
    Bert LSTM (X) layer 3 &0.23 &0.56 \\ \hline
    Bert LSTM (X) layer 4 &0.22 &0.56 \\ \hline
    Bert LSTM (y) layer 1 &0.01 &0.51 \\ \hline
    Bert LSTM (y) layer 2 &0.00 &0.50 \\ \hline
    Bert LSTM (y) layer 3 &0.00 &0.50 \\ \hline
    Bert LSTM (y) layer 4 &0.00 &0.50 \\ \hline
\end{tabular}
\end{table}

\textbf{Probability Distribution Model: }
We approach the probability distribution model while calculating probabilities of x-axis entities and y-axis values, using the distance from a x-axis entity to a y-axis value. Figure \ref{data_dis} shows the plotting of data distribution where the orange line refers to the negative distribution and the blue line refers to the positive distribution. We experiment this model in two ways - excluding and including punctuations from our dataset. After excluding or including all the punctuations, our dataset then contains 8487 positive and 1984 negative instances in the training set and 3026 positive and 548 negative instances in the validation set. 

\begin{figure}[hbt!]
    \centering
      \includegraphics[width=\linewidth]{data distribution.png}
      \caption{Data distribution of probability distribution model.}
      \label{data_dis}
    \end{figure}
    
\paragraph{Probability Distribution Model - excluding punctuations:}
Here, We remove all the punctuations before training the model. Table \ref{train_valid_pro_ex} contains the results of training and validation set using probability distribution model - excluding punctuations. We calculate the harmonic mean of F1-score using the positive and negative class F1-score. The harmonic mean of F1-score is 0.78 and 0.75 for training and validation instances respectively. Then we observe the ROC-AUC curves for both training \ref{roc_1} and validation set \ref{roc_2} and acquire the area under the ROC curve of 0.883 in the training set and 0.895 in the validation set. 

\begin{table}[!htb]
\caption{Stage 2 results of training and validation set using probability distribution model - excluding punctuations.}
\label{train_valid_pro_ex}
\footnotesize
\centering
\begin{tabular}{cccccp{3cm}p{2.2cm}}
    &Class &Precision &Recall &F1-score&Harmonic\,mean of\,F1-score&AUC-ROC \\ \hline
    \multicolumn{1}{c}{\multirow{2}{*}{Training set}}&0(-ve)&0.92&0.92&0.92&{\multirow{2}{*}{0.77}}&{\multirow{2}{*}{0.883}}\\
    \multicolumn{1}{c}{}&1 (+ve)&0.67&0.67&0.67&&\\ \hline
    \multicolumn{1}{c}{\multirow{2}{*}{Validation set}}&0(-ve)&0.93&0.93&0.93&{\multirow{2}{*}{0.75}}&{\multirow{2}{*}{0.895}}\\
    \multicolumn{1}{c}{}&1 (+ve)&0.63&0.63&0.63&&\\ \hline
\end{tabular}
\end{table}

\begin{figure}[hbt!]
    \centering
      \includegraphics[width=\linewidth]{ROC_Train_STAT_EX.PNG}
      \caption{ROC Curve for training instances excluding punctuations.}
      \label{roc_1}
    \end{figure}
    
\begin{figure}[hbt!]
    \centering
      \includegraphics[width=\linewidth]{ROC_Valid_STAT_EX.PNG}
      \caption{ROC Curve for validation instances excluding punctuations.}
      \label{roc_2}
    \end{figure}
    
\paragraph{Probability Distribution - including punctuations:}
Results show that the probability distribution model - excluding punctuations works much better than the transfer model. For further improvement of mapping x and y entities, here we experiment the same probability distribution model but including the punctuations. The results of the training and validation set are shown in Table \ref{train_valid_pro_in} where we obtain the harmonic mean of F1-score of 0.78 and 0.82 for training and validation set respectively. Similarly we observe the ROC-AUC curve of training and validation set in fingure \ref{roc_3} and \ref{roc_4} respectively, acquiring a better resulting area under the ROC curve of 0.908 in the training set and 0.914 in the validation set.

\begin{table}[!htb]
\caption{Stage 2 results of training and validation set using probability distribution model - including punctuations.}
\label{train_valid_pro_in}
\footnotesize
\centering
\begin{tabular}{cccccp{3cm}p{2.2cm}}
    &Class &Precision &Recall &F1-score&Harmonic\,mean of\,F1-score&AUC-ROC \\ \hline
    \multicolumn{1}{c}{\multirow{2}{*}{Training set}}&0(-ve)&0.94&0.94&0.94&{\multirow{2}{*}{0.84}}&{\multirow{2}{*}{0.908}}\\
    \multicolumn{1}{c}{}&1 (+ve)&0.76&0.76&0.76&&\\ \hline
    \multicolumn{1}{c}{\multirow{2}{*}{Validation set}}&0(-ve)&0.95&0.95&0.95&{\multirow{2}{*}{0.82}}&{\multirow{2}{*}{0.914}}\\
    \multicolumn{1}{c}{}&1 (+ve)&0.73&0.73&0.73&&\\ \hline
\end{tabular}
\end{table}

\begin{figure}[hbt!]
    \centering
      \includegraphics[width=\linewidth]{ROC_Train_STAT_In.PNG}
      \caption{ROC Curve for training instances including punctuations.}
      \label{roc_3}
    \end{figure}
    
\begin{figure}[hbt!]
    \centering
      \includegraphics[width=\linewidth]{ROC_Valid_STAT_In.PNG}
      \caption{ROC Curve for validation instances including punctuations.}
      \label{roc_4}
    \end{figure}

\textbf{X-X Distance and X-Y Displacement: }
We obtain this method by finding out the map of our targeted x and y entities, referring as x\textsubscript{t}, y\textsubscript{t}. For doing this, we use the displacement among all possible pairs from the feature set: S: x\textsubscript{t-1}, x\textsubscript{t}, x\textsubscript{t+1},  y\textsubscript{t-1}, y\textsubscript{t}, y\textsubscript{t+1}. The total number of features is 15. Here, we run the Support Vector Classifier (SVC) and Random Forest model while approaching this method. Then we compare these two models and choose the best one to attain the final result of the sub-task 2.

\paragraph{Support Vector Classifier (SVC) Model:}
We train the SVC model by configuring the Radial Basis Function (RBF) kernel and setting the parameter c to 6.0. The training and validation instances remain the same as previous models. For training and validation instances, we experiment the model as a probability using argmax calculation.
The results of the training and validation set for probability (argmax based calculation) are shown in table \ref{train_valid_svc} where we achieve the harmonic mean of F1-score of 0.81 and 0.86 for the training and validation set respectively. Then we observe the ROC-AUC of the probability (argmax) approach for both taining and validation set in figure \ref{argx1} and \ref{argx2}, which obtains 0.897 and 0.924 of the area under the ROC curve in the train and validation sets respectively.

\begin{table}[!htb]
\caption{Stage 2 results of training and validation set using SVC model.}
\label{train_valid_svc}
\footnotesize
\centering
\begin{tabular}{cccccp{3cm}p{2.2cm}}
    &Class &Precision &Recall &F1-score&Harmonic\,mean of\,F1-score&AUC-ROC \\ \hline
    \multicolumn{1}{c}{\multirow{2}{*}{Training set}}&0(-ve)&0.93&0.93&0.93&{\multirow{2}{*}{0.81}}&{\multirow{2}{*}{0.897}}\\
    \multicolumn{1}{c}{}&1 (+ve)&0.72&0.72&0.72&&\\ \hline
    \multicolumn{1}{c}{\multirow{2}{*}{Validation set}}&0(-ve)&0.96&0.96&0.96&{\multirow{2}{*}{0.86}}&{\multirow{2}{*}{0.924}}\\
    \multicolumn{1}{c}{}&1 (+ve)&0.78&0.78&0.78&&\\ \hline
\end{tabular}
\end{table}

\begin{figure}[hbt!]
    \centering
      \includegraphics[width=0.8\linewidth]{ROC_Train_SVC_NB.PNG}
      \caption{ROC Curve of training instances for probability - argmax based calculation using SVC.}
      \label{argx1}
    \end{figure}

\begin{figure}[hbt!]
    \centering
      \includegraphics[width=0.85\linewidth]{ROC_Valid_SVC_NB.PNG}
      \caption{ROC Curve of validation instances for probability - argmax based calculation using SVC.}
      \label{argx2}
    \end{figure}

\paragraph{Random Forest:} 
We set the random state to 111 and N estimator to 33 while training random forest approach. Therefore, we acquire the best results among all the other approaches discussed previously. The results of training and validation set are given in table \ref{train_valid_rf} where the obtained harmonic mean of F1-score is 0.85 and 0.84 in the training and validation set respectively. We observe the ROC-AUC curve for the training instances in figure \ref{rf_roc_train} and validation instances in figure \ref{rf_roc_valid}. Thus we calculate the area under the ROC curve which is 0.913 and 0.93 for the training and validation set respectively. 

\begin{table}[!htb]
\caption{Stage 2 results of training and validation set using Random Forest model.}
\label{train_valid_rf}
\footnotesize
\centering
\begin{tabular}{cccccp{3cm}p{2.2cm}}
    &Class &Precision &Recall &F1-score&Harmonic\,mean of\,F1-score&AUC-ROC \\ \hline
    \multicolumn{1}{c}{\multirow{2}{*}{Training set}}&0(-ve)&0.95&0.95&0.95&{\multirow{2}{*}{0.85}}&{\multirow{2}{*}{0.913}}\\
    \multicolumn{1}{c}{}&1 (+ve)&0.77&0.77&0.77&&\\ \hline
    \multicolumn{1}{c}{\multirow{2}{*}{Validation set}}&0(-ve)&0.96&0.96&0.96&{\multirow{2}{*}{0.84}}&{\multirow{2}{*}{0.93}}\\
    \multicolumn{1}{c}{}&1 (+ve)&0.77&0.77&0.77&&\\ \hline
\end{tabular}
\end{table}

\begin{figure}[hbt!]
    \centering
      \includegraphics[width=0.95\linewidth]{ROC_Train_RF.PNG}
      \caption{ROC Curve of training instances for random forest approach.}
      \label{rf_roc_train}
    \end{figure}

\begin{figure}[hbt!]
    \centering
      \includegraphics[width=0.9\linewidth]{ROC_Valid_RF.PNG}
      \caption{ROC Curve of validation instances for random forest approach.}
      \label{rf_roc_valid}
    \end{figure}

\paragraph{Comparion between SVC and Random Forest:} Table \ref{rf_svc_comp} shows the comparison of SVC and Random Forest based on several criteria such as F1-score, AUC-ROC, harmonic mean etc., helping us to choose the best performing model  in stage 2. Based on the results we choose the Random Forest model as it performs better than SVC and other previously discussed models. 

\begin{table}[!htb]
\caption{Comparison between SVC and random forest approach in stage 2}
\label{rf_svc_comp}
\centering
\begin{tabular}{|c|c|c|} \hline
    Criteria &SVC &Random Forest \\ \hline
    F1 (+ve) (validation) &0.78 &0.77 \\ \hline
    F1 (-ve) (validation) &0.96 &0.96 \\ \hline
    F1 (+ve) (training) &0.73 &0.77 \\ \hline
    F1 (-ve) (training) &0.93 &0.95 \\ \hline
    F1 (+ve) (Harmonic Mean of training and validation) &0.75 &0.76 \\ \hline
    F1 (-ve) (Harmonic Mean) &0.94 &0.95 \\ \hline
    AUC-ROC (validation) &0.924 &0.93 \\ \hline
    AUC-ROC (training) &0.897 &0.91 \\ \hline
    AUC-ROC (Harmonic Mean of training and validation) &0.904 &0.919 \\ \hline
\end{tabular}
\end{table}

\subsubsection{Final Results of Sub-Task 2: }
We train our dataset using random forest approach and tune the model with different seeds as shown in table \ref{rf_final_train}. Then we run our test set tuning with the same random seeds as train set and obtain the best results of average f1-score for positive class of 0.7794. The results of test set using random forest approach is given in table \ref{rf_final_test}. We also show the confusion matrix for both the train and test set in table \ref{cf_final}, showing the best and worst performing matrix on random seeds. 

\begin{table}[!htb]
\caption{Final results of stage 2 using random forest approach on training set}
\label{rf_final_train}
\footnotesize
\centering
\begin{tabular}{|p{1cm}|p{1.5cm}|p{1.3cm}|p{1.4cm}|p{1.5cm}|p{1.3cm}|p{1.4cm}|p{1.7cm}|}
Seed &Precision (0)&Recall (0)&F1-score (0)&Precision (1)&Recall (1)&F1-score (1)&AUC-ROC\\ \hline
111&0.9493&0.9493&0.9493&0.7694&0.7694&0.7694&0.918 \\ \hline
233&0.9494&0.9494&0.9494&0.7701&0.7701&0.7701&0.918 \\ \hline
254&0.9494&0.9494&0.9494&0.7697&0.7697&0.7697&0.918 \\ \hline
945&0.9494&0.9494&0.9494&0.7701&0.7701&0.7701&0.918 \\ \hline
607&0.9494&0.9494&0.9494&0.7697&0.7697&0.7697&0.918 \\ \hline
36&0.9493&0.9493&0.9493&0.7694&0.7694&0.7694&0.918 \\ \hline
\textbf{Avg}&\textbf{0.9494}&\textbf{0.9494}&\textbf{0.9494}&\textbf{0.7697}&\textbf{0.7697}&\textbf{0.7697}&\textbf{0.9180} \\ \hline
\end{tabular}
\end{table}

\begin{table}[!htb]
\caption{Final results of stage 2 using random forest approach on test set}
\label{rf_final_test}
\footnotesize
\centering
\begin{tabular}{|p{1cm}|p{1.5cm}|p{1.3cm}|p{1.4cm}|p{1.5cm}|p{1.3cm}|p{1.4cm}|p{1.7cm}|}
Seed &Precision (0)&Recall (0)&F1-score (0)&Precision (1)&Recall (1)&F1-score (1)&AUC-ROC\\ \hline
111&0.9495&0.9491&0.9493&0.7787&0.7801&0.7794&0.917 \\ \hline
233&0.9495&0.9491&0.9493&0.7787&0.7801&0.7794&0.917 \\ \hline
254&0.9495&0.9491&0.9493&0.7787&0.7801&0.7794&0.917 \\ \hline
945&0.9495&0.9491&0.9493&0.7787&0.7801&0.7794&0.917 \\ \hline
607&0.9495&0.9491&0.9493&0.7787&0.7801&0.7794&0.917 \\ \hline
36&0.9495&0.9491&0.9493&0.7787&0.7801&0.7794&0.917 \\ \hline
\textbf{Avg}&\textbf{0.9495}&\textbf{0.9491}&\textbf{0.9493}&\textbf{0.7787}&\textbf{0.7801}&\textbf{0.7794}&\textbf{0.9170} \\ \hline
\end{tabular}
\end{table}

\begin{table}[!htb]
\caption{Confusion matrix of the final results of stage 2}
\label{cf_final}
\footnotesize
\centering
\begin{tabular}{cccccc}
    &Seed &TN(0,0) &FP(0, 1)&FN (1, 0)&TP(1, 1) \\ \hline
    \multicolumn{1}{c}{\multirow{2}{*}{Training set}}&111&10929&584&	584&1948\\
    \multicolumn{1}{c}{}&233&10931&582&582&1950\\ \hline
    \multicolumn{1}{c}{\multirow{2}{*}{Test set}}&111&2368&127&126&447\\
    \multicolumn{1}{c}{}&233&2368&127&126&447\\ \hline
\end{tabular}
\end{table}

\subsubsection{Experimental Analysis of Stage 3: }
After successfully extracting the x and y-axis entities in stage 1, and mapping the x-axis entity to its corresponding y-axis value in stage 2, here we try to predict the suitable chart type. In order to generate a chart out of a human written text, we are to make sure which chart is best suited for the particular text. Thus we have named this task as stage 3 - predicting the suitable chart type. 

We have created a corpora with 717 samples, suitable to generate charts from. We have manually labeled all the data and identified that the bar charts can be generated from each of the samples. Thus for the chart type prediction task, we exclude bar charts and run our classifier on pie and line charts only. Our model predicts whether a given text input can be generated as a line chart or a pie chart. For this task we use a model using the combination of fastText and LSTM. We train the model in order to find out the texts suitable for pie chart type at first and for the line chart type next. We measure the performance of our model in terms of specificity, sensitivity or recall, MCC and AUC-ROC, as shown in the table \ref{s3_final}. We obtain the results while tuning the parameters as - lstm layer: 128, 128, dense layer: 512, 1, class weight: 0:0.2, 1:1, text sequence length: 200 and optimizer: RMSprop for the both pie and line charts. To show the prediction results in a brief, we exhibit the confusion matrix for the both pie and line charts in table \ref{s3_final_cf}. We have plotted TPR vs FPR graphs for the prediction of pie and line chart type in train, validation and test sets in the figures \ref{pie_train}, \ref{pie_valid}, \ref{pie_test}, \ref{line_train}, \ref{line_valid} and \ref{line_test} respectively.

\begin{figure}[hbt!]
    \centering
      \includegraphics[width=0.85\linewidth]{pie_train.jpg}
      \caption{True positive rate vs false positive rate of pie chart type prediction in the training set.}
      \label{pie_train}
    \end{figure}

\begin{figure}[hbt!]
    \centering
      \includegraphics[width=0.85\linewidth]{pie_valid.jpg}
      \caption{True positive rate vs false positive rate of pie chart type prediction in the validation set.}
      \label{pie_valid}
    \end{figure}

\begin{figure}[hbt!]
    \centering
      \includegraphics[width=0.85\linewidth]{pie_test.jpg}
      \caption{True positive rate vs false positive rate of pie chart type prediction in the test set.}
      \label{pie_test}
    \end{figure}

\begin{figure}[hbt!]
    \centering
      \includegraphics[width=0.85\linewidth]{line_train.jpg}
      \caption{True positive rate vs false positive rate of line chart type prediction in the training set.}
      \label{line_train}
    \end{figure}

\begin{figure}[hbt!]
    \centering
      \includegraphics[width=0.85\linewidth]{line_valid.jpg}
      \caption{True positive rate vs false positive rate of line chart type prediction in the validation set.}
      \label{line_valid}
    \end{figure}

\begin{figure}[hbt!]
    \centering
      \includegraphics[width=0.85\linewidth]{line_test.jpg}
      \caption{True positive rate vs false positive rate of line chart type prediction in the test set.}
      \label{line_test}
    \end{figure}

\textbf{Chart Type Prediction for Pie Charts: } 
For pie chart type, we set the batch size to 128 and the learning rate to 4e-4. As we have a highly imbalanced dataset, we achieve good enough results in terms of MCC, scoring 22\% in the test set as shown in table \ref{s3_final}. The obtained AUC for pie charts is 0.64 in the test set. We avail a better result in terms of recall or sensitivity of 0.94 in the training set, 0.71 in the validation set and 0.75 in the test set respectively.
\textbf{Chart Type Prediction for Line Charts:}
We set the batch size to 256 and the learning rate remains as default to 1e-3 for the line charts. Here in table \ref{s3_final}, we avail outstanding results in terms of AUC scoring 96\% in the training set, 98\% in the validation set and over 90\% in the test set respectively. Our obtained MCC in the train, validation and test sets is 0.96, 0.92 and 0.51 which is a better score than the prediction of pie charts. 
\begin{table}[!htb]
\caption{Stage 3 results for pie and line charts}
\label{s3_final}
\footnotesize
\centering
\begin{tabular}{p{1.3cm}p{2.2cm}ccp{1.0cm}p{1.0cm}}
    &&Specificity &Sensitivity&MCC&AUC\\ \hline
    \multicolumn{1}{c}{\multirow{3}{*}{Pie Chart}}&Training set&0.742&0.944&0.51&0.86\\
    \multicolumn{1}{c}{}&Validation set&0.6945&0.714&0.32&0.66\\ 
    \multicolumn{1}{c}{}&Test set&0.573&0.75&0.22&0.64\\ \hline
    \multicolumn{1}{c}{\multirow{3}{*}{Line Chart}}&Training set&0.9634&0.963&0.96&0.96\\
    \multicolumn{1}{c}{}&Validation set&0.990&0.933&0.92&0.98\\ 
    \multicolumn{1}{c}{}&Test set&0.893&0.733&0.51&0.91\\ \hline
\end{tabular}
\end{table}

\begin{table}[!htb]
\caption{Confusion matrix of stage 3}
\label{s3_final_cf}
\footnotesize
\centering
\begin{tabular}{p{1.3cm}p{2.2cm}p{1.2cm}p{1.0cm}p{1.0cm}p{1.0cm}p{1.5cm}p{1.5cm}}
    && TN (0,0) & FP (0,1) & FN (1,0) & TP (1,1) &positive instances &negative instances\\ \hline
    \multicolumn{1}{c}{\multirow{3}{*}{Pie Chart}}&Training set&291&101&4&68&392&72\\
    \multicolumn{1}{c}{}&Validation set&66&29&6&15&95&21\\ 
    \multicolumn{1}{c}{}&Test set&67&50&5&15&117&20\\ \hline
    \multicolumn{1}{c}{\multirow{3}{*}{Line Chart}}&Training set&395&15&2&52&410&54\\
    \multicolumn{1}{c}{}&Validation set&100&1&1&14&101&15\\ 
    \multicolumn{1}{c}{}&Test set&109&13&4&11&122&15\\ \hline
\end{tabular}
\end{table}

\subsubsection{Overall Performance and Discussion: }
In order to discuss the overall performance of our work, we have created a pipeline same as shown in figure \ref{archi}. Our pipeline merges all the stages of our work and outputs the results we have already discussed and shown in this section. After obtaining the final results, we have checked for all possible errors for each of the stages. The frequency and the cumulative frequency of error count for each of the stages is shown in figure \ref{free} and \ref{cum} respectively, where we have observed that the green line referring to the stage 3 errors are comparatively more than stage 1 and 2. One of the possible reasons for occurring more numbers of errors in stage 3 can be because of our small corpus, where the number of instances \ref{s3_final_cf} are very less than stage 1 \ref{1_final} or 2 \ref{cf_final}. Thus we believe further improvement is possible in stage 3.

\begin{table}[!htb]
\caption{Error count of test set for stage 1, 2 and 3.}
\label{Error_count}
\centering
\begin{tabular}{|c|c|c|c|} \hline
    Error Count &Stage 1 &Stage 2&Stage 3 \\ \hline
    0&37&9&3\\ \hline
    1&30&23&16 \\ \hline
    2&15&15&19 \\ \hline
    3&17&11&15 \\ \hline
    4&12&21&9 \\ \hline
    5&4&15&20 \\ \hline
    6&7&12&20 \\ \hline
    7&3&4&7 \\ \hline
    8&2&6&6 \\ \hline
    9&3&6&2 \\ \hline
    10&2&2&7 \\ \hline
    11&1&1&1 \\ \hline
    12&1&3&2 \\ \hline
    13&0&0&1 \\ \hline
    14&1&1&1 \\ \hline
    15&1&1&0 \\ \hline
    16&0&0&1 \\ \hline
    17&1&1&0 \\ \hline
    18&0&3&3 \\ \hline
    19&0&0&1 \\ \hline
    20&0&1&1 \\ \hline
    21&0&0&0 \\ \hline
    22&0&2&2 \\ \hline
    23&0&0&0 \\ \hline
    24&0&0&0 \\ \hline
    25&0&0&0 \\ \hline
\end{tabular}
\end{table}

\begin{figure}[hbt!]
    \centering
      \includegraphics[width=\linewidth]{Frequency.png}
      \caption{Frequency of error count of stage 1, stage 2 and stage 3}
      \label{free}
    \end{figure}

\begin{figure}[hbt!]
    \centering
      \includegraphics[width=\linewidth]{Cumulative.png}
      \caption{Cumulative frequency of error count of stage 1, stage 2 and stage 3}
      \label{cum}
    \end{figure}

\begin{figure}[hbt!]
    \centering
      \includegraphics[width=\linewidth]{2StageSep.png}
      \caption{Error shown as bars for each test sample of stage 1 and stage 2.}
      \label{2stage}
    \end{figure}

\begin{figure}[hbt!]
    \centering
      \includegraphics[width=\linewidth]{3StageSep.png}
      \caption{Error shown as bars for each test sample of stage 1, stage 2 and stage 3.}
      \label{3stage}
    \end{figure}
    
\begin{table}[!htb]
\caption{Overall error count by conditional bypassing of stage 2.}
\label{Error_count_bypass}
\centering
\begin{tabular}{|c|c|c|c|} \hline
    Error Count &Stage 1 &Stage 2&Stage 3\\ \hline
    0& 37&	31&	14\\ \hline
    1& 30&	11&	22\\ \hline
    2& 15&	12&12\\ \hline
    3&	17&	11&	10\\ \hline
    4&	12&	20&	11\\ \hline
    5&	4&	14&	20\\ \hline
    6&	7&	10&	16\\ \hline
    7&	3&	3&	5\\ \hline
    8&	2&	5&	6\\ \hline
    9&	3&	5&	2\\ \hline
    10&	2&	3&	6\\ \hline
    11&	1&	1&	2\\ \hline
    12&	1&	2&	2\\ \hline
    13&	0&	0&	0\\ \hline
    14&	1&	1&	1\\ \hline
    15&	1&	1&	0\\ \hline
    16&	0&	0&	1\\ \hline
    17&	1&	1&	0\\ \hline
    18&	0&	3&	3\\ \hline
    19&	0&	0&	1\\ \hline
    20&	0&	1&	1\\ \hline
    21&	0&	0&	0\\ \hline
    22&	0&	2&	2\\ \hline
\end{tabular}
\end{table}

\begin{figure}[hbt!]
    \centering
      \includegraphics[width=0.85\linewidth]{CumilitiveFrequency_Bypass.png}
      \caption{Cumulative error frequency of stage 1, 2 and 3 by conditional bypassing of stage 2.}
      \label{error_Cu_by}
    \end{figure}

\begin{figure}[hbt!]
    \centering
      \includegraphics[width=0.85\linewidth]{Frequency_Bypass.png}
      \caption{Error frequency of stage 1, 2 and 3 by conditional bypassing of stage 2.}
      \label{error_fre_by}
    \end{figure}

\begin{figure}[hbt!]
    \centering
      \includegraphics[width=0.85\linewidth]{Stage(1,2)Error_Bypass.png}
      \caption{Error shown as bars for each test sample of stage 1 and stage 2 by conditional bypassing of stage 2.}
      \label{1_2_error_bypass}
    \end{figure}

\begin{figure}[hbt!]
    \centering
      \includegraphics[width=0.85\linewidth]{Stage(1,2,3)Error_Bypass.png}
      \caption{Error shown as bars for each test sample of stage 1, 2 and 3 by conditional bypassing of stage 2.}
      \label{1_2_3_error_bypass}
    \end{figure}

To be more clear about the error frequency, we have plotted a bar graph for all the stages shown in figure \ref{3stage}. This graph \ref{3stage} includes bars for each of the samples of the test set, 137 samples in total. We have differentiated the errors of bars by color such as; blue bars for the errors of stage 1, red for stage 2 and green for stage 3. Here we can see that nearly all the samples include at least some errors, where errors occurring in the stage 3 exist in most of the samples. We have also observed while experimenting our model for stage 3 that stage 3 performs significantly lower than stage 1 or 2. Therefore we have excluded stage 3 to evaluate the errors occurring in stage 1 and 2, figure shown in \ref{2stage}. Here we obtain much better results for the samples that include zero error or only one or two errors while excluding stage 3 out of our evaluation. As each of the stages are independent, stage 2 performs better in some samples yet underperforms in some. For stage 1, we obtain satisfactory results in tracing errors as there exist many samples occurring only one or two errors and even zero errors. 

In the table \ref{example_1} and \ref{example_2} we show two sample input and their output generated by our technique.

\begin{table}[!htb]
\caption{Text input and the generated output (Partial Correct) by our model.}
\label{example_1}
\centering
\begin{tabular}{c|c|p{8cm}}
    \multirow{4}{*}{Input}&\multirow{4}{*}{Sample Text}&Multi - unit residential dwellings typically break down as follows : acquisition costs , 7 \% ; site improvement costs , 8 \% ; labour costs , 27 \% ; materials costs , 33 \% ; finance costs , 3 \% ; administrative costs , 17 \% ; and marketing costs , 5 \%\\ \hline
    \multicolumn{1}{c}{\multirow{4}{*}{Output}}&X-Labels& ['acquisition', 'site improvement', 'labour', 'materials', 'finance', 'administrative', 'and marketing']\\ 
    \multicolumn{1}{c}{}&Y-Labels& ['7', '8', '27', '33', '3', '17', '5']\\
    \multicolumn{1}{c}{}&Chart Type&['bar']\\ \hline
\end{tabular}
\end{table}

\begin{table}[!htb]
\caption{Text input and the generated output (Fully Correct) by our model.}
\label{example_2}
\centering
\begin{tabular}{c|c|p{8cm}}
    \multirow{8}{*}{Input}&\multirow{8}{*}{Sample Text}&Mr . Jamal worked in the Meteorological Department for 8 years . He noticed a strange thing in recent times . On certain days of the month , the weather varied strongly . He wrote down the information to make a pattern of the event . The information of the paper is as follows : on the 3rd day of the month the temperature is 36 degrees Celsius , 7th day is 45 degrees Celsius , 9th day is 18 degrees Celsius , 11th day is 21 degrees Celsius , 17th day is 9 degrees Celsius , 19th day is 45 degrees Celsius , 21st day is 36 degrees Celsius , 27th day is 21 degrees Celsius and 29th day is 45 degrees Celsius . He finds a weird pattern in these dates and makes a report and sends it to his senior officer .\\ \hline
    \multicolumn{1}{c}{\multirow{4}{*}{Output}}&X-Labels& ['3rd day', '7th day', '9th day', '11th day', '17th day', '19th day', '21st day', '27th day', '29th day']\\ 
    \multicolumn{1}{c}{}&Y-Labels&  ['36', '45', '18', '21', '9', '45', '36', '21', '45']\\
    \multicolumn{1}{c}{}&Chart Type&['bar', 'Line']\\ \hline
\end{tabular}
\end{table}
\end{comment}
